Algebraic geometry over the residue field of the infinite place

Nikolai Durov introduced the theory of generalized rings and schemes to study Arakelov geometry in an alternative algebraic framework, and introduced the residue field at the infinite place. We show an elementary algebraic approach to modules and algebras over this object, define prime congruences, show that the polynomial ring of n variables is of Krull dimension n, and derive a prime decomposition theorem for these primes.

==> defs.tex <==
\hyphenation{iso-mor-phisms pa-pers}

% Nice script font. My reference due to Ron Donagi and Paul Aspinwall
%
\DeclareFontFamily{U}{rsf}{}
\DeclareFontShape{U}{rsf}{m}{n}{
  <5> <6> rsfs5 <7> <8> <9> rsfs7 <10-> rsfs10}{}
\DeclareMathAlphabet{\mathscr}{U}{rsf}{m}{n}

% Gothic font
\DeclareMathAlphabet{\mathgth}{U}{euf}{m}{n}

\DeclareFontFamily{U}{cyr}{}
\DeclareFontShape{U}{cyr}{m}{n}{
  <5> wncyr5 <6> wncyr6 <7> wncyr7 <8> wncyr8 <9> wncyr9 <10-> wncyr10}{}
\DeclareMathAlphabet{\mathcyr}{U}{cyr}{m}{n}

% Cyrillic font, for the TS group
\input cyracc.def

\newcommand{\Sha}{\mathcyr{\cyracc Sh}}

%\DeclareMathAlphabet{\mathbb}{U}{bbold}{m}{n}
% \DeclareSymbolFont{bbold}{U}{bbold}{m}{n}
% \DeclareSymbolFontAlphabet{\mathbb}{bbold}

%%%%%%%%%%%%%%%%%%%%%%%%
% there should be a \makeatletter-free way of changing this, but I can't find
% it...

\makeatletter
\def\operator@font{\sf}
\makeatother

\newcommand{\sbt}{{\scalebox{0.5}{\textbullet}}}
\setlength{\unitlength}{1 true in}
\newcommand{\eps}{\epsilon}
\newcommand{\lieg}{\mathfrak{g}}
\newcommand{\gA}{\mathgth{a}}
\newcommand{\gB}{\mathgth{b}}
\newcommand{\gF}{\mathgth{F}}
\newcommand{\gG}{\mathgth{G}}
\newcommand{\gM}{\mathgth{m}}
\newcommand{\gN}{\mathgth{N}}
\newcommand{\gO}{\mathgth{o}}
\newcommand{\gP}{\mathgth{p}}
\newcommand{\gQ}{\mathgth{q}}
\newcommand{\gR}{\mathgth{r}}
\newcommand{\gU}{\mathgth{U}}
\newcommand{\gV}{\mathgth{V}}
\newcommand{\gog}{\mathgth{g}}
\newcommand{\gh}{\mathgth{h}}
\newcommand{\gn}{\mathgth{n}}
\newcommand{\gm}{\mathgth{m}}
\newcommand{\Ab}{\mathgth{Ab}}
\newcommand{\gVect}{\mathgth{Vect}}
\newcommand{\hA}{\hat{A}}
\newcommand{\cA}{{\mathscr A}}
\newcommand{\cB}{{\mathscr B}}
\newcommand{\sA}{{\mathcal A}}
\newcommand{\sB}{{\mathcal B}}
\newcommand{\sC}{{\mathcal C}}
\newcommand{\sD}{{\mathcal D}}
\newcommand{\sN}{{\mathcal N}}
\newcommand{\sT}{{\mathcal T}}
\newcommand{\sDG}{{\mathcal{DG}}}
\newcommand{\sK}{{\mathcal K}}
\newcommand{\usK}{{\underline {\mathcal K}}}
\newcommand{\sL}{{\mathcal L}}
\newcommand{\sP}{{\mathcal P}}
\newcommand{\sX}{{\mathgth X}}
\newcommand{\sY}{{\mathgth Y}}
\newcommand{\Ug}{{\mathbf U}\gog}
\newcommand{\Sg}{{\mathbf S}\gog}
\newcommand{\Sn}{{\mathbf S}\gn}
\newcommand{\UV}{{\mathbf U}V}
\newcommand{\TV}{{\mathbf T}V}
\newcommand{\SV}{{\mathbf S}V}
\newcommand{\cC}{{\mathscr C}}
\newcommand{\cE}{{\mathscr E}}
\newcommand{\cF}{{\mathscr F}}
\newcommand{\cG}{{\mathscr G}}
\newcommand{\coH}{{\mathscr H}}
\newcommand{\cI}{{\mathscr I}}
\newcommand{\cJ}{{\mathscr J}}
\newcommand{\cK}{{\mathscr K}}
%\newcommand{\cL}{{\mathscr L}}
\newcommand{\cM}{{\mathscr M}}
\newcommand{\cN}{{\mathscr N}}
\newcommand{\cO}{{\mathscr O}}
\newcommand{\OO}{{\mathcal O}}
\newcommand{\cP}{{\mathscr P}}
\newcommand{\cQ}{{\mathscr Q}}
%\newcommand{\cR}{{\mathscr R}}
\newcommand{\cS}{{\mathscr S}}
\newcommand{\cT}{{\mathscr T}}
\newcommand{\cU}{{\mathscr U}}
\newcommand{\cZ}{{\mathscr Z}}
\newcommand{\tcU}{{\tilde{\cU}}}
\newcommand{\cV}{{\mathscr V}}
\newcommand{\cX}{{\mathscr X}}
\newcommand{\bA}{{\bar{A}}}
\newcommand{\ba}{{\bar{a}}}
\newcommand{\bB}{{\bar{B}}}
\newcommand{\bb}{{\bar{b}}}
\newcommand{\bC}{{\bar{C}}}
\newcommand{\bc}{{\bar{c}}}
\newcommand{\bE}{{\overline{E}}}
\newcommand{\bF}{{\overline{F}}}
\newcommand{\bG}{{\overline{G}}}
\newcommand{\bV}{{\overline{V}}}
\newcommand{\bJ}{{\bar{J}}}
\newcommand{\bK}{{\bar{K}}}
\newcommand{\bM}{{\bar{M}}}
\newcommand{\bN}{{\overline{N}}}
\newcommand{\bT}{{\overline{T}}}
\newcommand{\bZ}{{\overline{Z}}}
\newcommand{\SN}{{\mathbf{S^*N}}}
\newcommand{\bR}{{\bar{R}}}
\newcommand{\bX}{{\overline{X}}}
\newcommand{\bY}{{\overline{Y}}}
\newcommand{\bW}{{\overline{W}}}
\newcommand{\bS}{{\overline{S}}}
\newcommand{\bH}{{\mathbf{H}}}
\newcommand{\balpha}{{\bar{\alpha}}}
\newcommand{\bbeta}{{\bar{\beta}}}
\newcommand{\bdel}{{\bar{\del}}}
\newcommand{\bg}{{\bar{g}}}
\newcommand{\bif}{{\bar{f}}}
\newcommand{\bi}{{\bar{i}}}
\newcommand{\bj}{{\bar{j}}}
\newcommand{\bp}{{\bar{p}}}
\newcommand{\bq}{{\bar{q}}}
\newcommand{\bs}{{\bar{s}}}
\newcommand{\bw}{{\bar{w}}}
\newcommand{\bphi}{{\bar{\phi}}}
\newcommand{\bpi}{{\bar{\pi}}}
\newcommand{\bcF}{{\overline{\cF}}}
\newcommand{\bcG}{{\overline{\cG}}}
\newcommand{\ccH}{{\mathscr H}}
\newcommand{\tF}{\tilde{F}}
\newcommand{\tG}{\tilde{G}}
\newcommand{\tH}{\tilde{H}}
\newcommand{\tM}{\tilde{M}}
\newcommand{\tN}{\tilde{N}}
\newcommand{\tX}{\tilde{X}}
\newcommand{\tY}{\tilde{Y}}
\newcommand{\tcF}{\tilde{\cF}}
\newcommand{\tcG}{\tilde{\cG}}
\newcommand{\tcI}{\tilde{\cI}}
\newcommand{\hcB}{\widehat{\cB\,\,}\!\!}
\newcommand{\hcC}{\widehat{\cC}}
\newcommand{\vC}{\check{C}}
\newcommand{\vH}{\check{H}}
\newcommand{\dE}{{E^{\cdot}}}
\newcommand{\dcE}{{\cE^{\cdot}}}
\newcommand{\dF}{{F^{\cdot}}}
\newcommand{\dFp}{{F'}^{\cdot}}
\newcommand{\dFpp}{{F''}^{\cdot}}
\newcommand{\dG}{G^{\cdot}}
\newcommand{\dH}{H^{\cdot}}
\newcommand{\dI}{I^{\cdot}}
\newcommand{\dJ}{J^{\cdot}}
\newcommand{\dL}{L^{\cdot}}
\newcommand{\dP}{P^{\cdot}}
%\newcommand{\dX}{X^{\cdot}}
\newcommand{\dXp}{{X'}^{\cdot}}
\newcommand{\dXpp}{{X''}^{\cdot}}
%\newcommand{\dY}{Y^{\cdot}}
\newcommand{\dYp}{{Y'}^{\cdot}}
\newcommand{\dYpp}{{Y''}^{\cdot}}
\newcommand{\dU}{{U^{\cdot}}}
\newcommand{\dUp}{{U'}^{\cdot}}
\newcommand{\dUchk}{{{U^\cdot}^{\chk}}}
\newcommand{\dcI}{\cI^{\cdot}}
\newcommand{\dcJ}{\cJ^{\cdot}}
\newcommand{\FMYX}{\Phi_{Y\ra X}}
\newcommand{\FMXX}{\Phi_{X\ra X}}
\newcommand{\FMXY}{\Phi_{X\ra Y}}
\newcommand{\FMZY}{\Phi_{Z\ra Y}}
\newcommand{\FMZX}{\Phi_{Z\ra X}}
\newcommand{\FMYZ}{\Phi_{Y\ra Z}}
\newcommand{\FMXZ}{\Phi_{X\ra Z}}
\newcommand{\fmYX}{\phi_{Y\ra X}}
\newcommand{\fmXY}{\phi_{X\ra Y}}
\newcommand{\fmXX}{\phi_{X\ra X}}
\newcommand{\fmYY}{\phi_{Y\ra Y}}
\newcommand{\fmXM}{\phi_{X\ra M}}
\newcommand{\fmYZ}{\phi_{Y\ra Z}}
\newcommand{\fmXZ}{\phi_{X\ra Z}}
\newcommand{\FMXM}{\Phi_{X\ra M}}
\newcommand{\FMMX}{\Phi_{M\ra X}}

\newcommand{\dR}{{\mathsf dR}}
\newcommand{\dr}{{\mathsf d}}
\newcommand{\orb}{{\mathsf{orb}}}
\newcommand{\even}{{\mathsf{even}}}
\newcommand{\odd}{{\mathsf{odd}}}
\newcommand{\perf}{{\mathsf{perf}}}
\newcommand{\inertia}{{\mathsf{i}}}
\newcommand{\mycap}{\smallfrown}
\newcommand{\mycup}{\smallsmile}
\newcommand{\HKR}{{\mathsf{HKR}}}
\newcommand{\PBW}{{\mathsf{PBW}}}
\newcommand{\sHom}{\underline{\mathsf{Hom}}}
\newcommand{\sTor}{\underline{\mathsf{Tor}}}
\newcommand{\RsHom}{{\R\sHom}}
\newcommand{\THom}{{2\mbox{-}\mathsf{Hom}}}
\newcommand{\DGHom}{{\mathsf{DG}\mbox{-}\mathsf{Hom}}}
\newcommand{\sExt}{\underline{\mathsf{Ext}}}
\newcommand{\sEnd}{\underline{\mathsf{End}}}
\newcommand{\RsEnd}{\underline{\mathbf{R}\mathsf{End}}}
\newcommand{\bProj}{\mathbf{Proj}}
\newcommand{\con}{N^\chk}
%\newcommand{\D}{{\mathbf D}_{\mathsf{coh}}^b}
\newcommand{\D}{{\mathbf D}}
\newcommand{\DG}{{\mathbf{DG}}}
\newcommand{\PreD}{\tilde{\mathbf D}}
%\newcommand{\Dp}{{\mathbf D}_{\mathsf{coh}}^+}
\newcommand{\Dm}{{\mathbf D}_{\mathsf{coh}}^-}
\newcommand{\Dn}{{\mathbf D}_{\mathsf{coh}}}
\newcommand{\K}{{\mathbf K}_{\mathsf{coh}}^b}
\newcommand{\Kp}{{\mathbf K}_{\mathsf{coh}}^+}
\newcommand{\Km}{{\mathbf K}_{\mathsf{coh}}^-}
\newcommand{\Kn}{{\mathbf K}_{\mathsf{coh}}}
\newcommand{\chk}{{\scriptscriptstyle\vee}}
\newcommand{\R}{\mathbf{R}}
\newcommand{\Na}{{\nabla}}
\newcommand{\Ld}{\mathbf{L}}
\newcommand{\lotimes}{\stackrel{\Ld}{\otimes}}
\newcommand{\Ltimes}{\underline{\underline{\times}}}
%\newcommand{\lotimes}{\underline{\otimes}}
\newcommand{\et}{{\mathsf{\acute{e}t}}}
\newcommand{\an}{{\mathsf{an}}}
\newcommand{\At}{{\mathsf{at}}}
\newcommand{\op}{{\mathsf{op}}}
\newcommand{\pt}{{\mathsf{pt}}}
\newcommand{\tors}{{\mathsf{tors}}}
\newcommand{\free}{{\mathsf{free}}}
\newcommand{\Kt}{{\mathsf{K3}}}
\newcommand{\bbk}{\mathbf{k}}
\newcommand{\bbL}{\mathbb{L}}
\newcommand{\bbE}{\mathbb{E}}
\newcommand{\blob}{{\scriptscriptstyle\bullet}}
\newcommand{\Kw}{K^{\scriptscriptstyle{\wedge}}_\blob}
\newcommand{\Ko}{K^{\scriptscriptstyle{\otimes}}_\blob}
\newcommand{\bone}{{\mathbf 1}}
\newcommand{\triv}{{\mathbf{triv}}}
\newcommand{\Duflo}{{\mathrm{Duflo}}}
\newcommand{\bL}{{\mathbb{L}}}
\newcommand{\Gm}{{\mathbb G}_m}
\renewcommand{\S}{{\mathbb{S}}}
\DeclareMathOperator{\Rep}{Rep}
\DeclareMathOperator{\Ch}{Ch}
\DeclareMathOperator{\ChInj}{ChInj}
\DeclareMathOperator{\Tr}{Tr}
\DeclareMathOperator{\sTr}{Tr}
\DeclareMathOperator{\Nat}{Nat}
\DeclareMathOperator{\Cone}{Cone}
\DeclareMathOperator{\Tors}{Tors}
\DeclareMathOperator{\Split}{Spl}
\DeclareMathOperator{\Spec}{Spec}
\DeclareMathOperator{\Ann}{Ann}
\DeclareMathOperator{\Ass}{Ass}
\DeclareMathOperator{\ExFun}{ExFun}
\DeclareMathOperator{\bExFun}{ExFun^+}
\DeclareMathOperator{\Prex}{Prex}
\DeclareMathOperator{\Der}{Der}
\DeclareMathOperator{\dt}{depth}
\DeclareMathOperator{\Aut}{Aut}
\DeclareMathOperator{\Obs}{Obs}
\DeclareMathOperator{\Supp}{Supp}
\newcommand{\Hom}{{\mathsf{Hom}}}
\DeclareMathOperator{\End}{End}
\DeclareMathOperator{\RHom}{RHom}
\DeclareMathOperator{\Tor}{Tor}
\DeclareMathOperator{\Tot}{Tot}
\DeclareMathOperator{\Ker}{Ker}
\DeclareMathOperator{\Maps}{Maps}
\DeclareMathOperator{\Coker}{Coker}
\DeclareMathOperator{\Proj}{Proj}
\DeclareMathOperator{\Pic}{Pic}
\DeclareMathOperator{\ParPic}{ParPic}
\DeclareMathOperator{\CaCl}{CaCl}
\DeclareMathOperator{\PGL}{PGL}
\DeclareMathOperator{\GL}{GL}
\DeclareMathOperator{\PSL}{PSL}
\DeclareMathOperator{\SL}{SL}
\DeclareMathOperator{\Td}{td}
\DeclareMathOperator{\ch}{ch}
\DeclareMathOperator{\ord}{ord}
\DeclareMathOperator{\imag}{Im}
\DeclareMathOperator{\id}{id}
\DeclareMathOperator{\ev}{ev}
\DeclareMathOperator{\coev}{coev}
\DeclareMathOperator{\Id}{Id}
\DeclareMathOperator{\topsp}{sp}
\DeclareMathOperator{\chr}{char}
\DeclareMathOperator{\card}{card}
\DeclareMathOperator{\Cl}{Cl}
\DeclareMathOperator{\Br}{Br}
\DeclareMathOperator{\FM}{FM}
\DeclareMathOperator{\NS}{NS}
\DeclareMathOperator{\Ob}{obj}
\DeclareMathOperator{\lgt}{length}
\DeclareMathOperator{\rk}{rk}
\DeclareMathOperator{\Ext}{Ext}
\DeclareMathOperator{\Spinc}{Spin^c}
\DeclareMathOperator{\rad}{rad}
\DeclareMathOperator{\td}{tr.d.}
\DeclareMathOperator{\hgt}{ht}
\DeclareMathOperator{\codim}{codim}
\DeclareMathOperator{\sym}{Sym}
\DeclareMathOperator{\Crit}{Crit}
\DeclareMathOperator{\dSt}{dSt}
\newcommand{\Tc}{{\mathbb{T}^c}}
\newcommand{\T}{\mathbb{T}}
\newcommand{\U}{\mathbf{U}}
\newcommand{\CN}{\mathbf{CN}}
\newcommand{\sH}{\mathbf{H}}
\newcommand{\adjoint}{\dashv}
\newcommand{\triangulated}{\mathsf{triangulated}}
\newcommand{\red}{\mathsf{red}}
\newcommand{\DSch}{\mathgth{DSch}}
\newcommand{\ra}{\rightarrow}
\newcommand{\Ra}{\Rightarrow}
\newcommand{\lra}{\longrightarrow}
\newcommand{\contract}{\lrcorner}
\newcommand{\raiso}{\stackrel{\sim}{\longrightarrow}}
\newcommand{\inj}{\hookrightarrow}
\newcommand{\surj}{\twoheadrightarrow}
\newcommand{\lsurj}{\twoheadleftarrow}
\newcommand{\imp}{~\Rightarrow~}
\newcommand{\scdot}{{\,\cdot\,}}
\newcommand{\rder}{{R}}
\newcommand{\rn}{\mathbf{R}}
\newcommand{\qn}{\mathbf{Q}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\G}{\mathbf{G}}
\newcommand{\Q}{\mathbf{Q}}
\newcommand{\Z}{\mathbf{Z}}
\newcommand{\gMod}{\mathgth{Mod}}
\newcommand{\gCoh}{\mathgth{Coh}}
\newcommand{\gEns}{\mathgth{Ens}}
\newcommand{\gCat}{\mathgth{Cat}}
\newcommand{\gSch}{\mathgth{Sch}}
\newcommand{\gQCoh}{\mathgth{Qcoh}}
\newcommand{\mx}{\mathgth{m}}
\newcommand{\iso}{\cong}
\newcommand{\Cech}{\v{C}ech }
\newcommand{\hc}{\check{H}}
\newcommand{\specialize}{\leadsto}
\newcommand{\eqv}{~\Leftrightarrow~}
\newcommand{\af}{\mathbf{A}}
\newcommand{\pj}{\mathbf{P}}
\newcommand{\img}{\mathsf{Im}~}
\newcommand{\st}{~|~}\newcommand{\fTd}{{\mathsf{fTd}}}
\newcommand{\homeo}{\approx}
\newcommand{\lineq}{\sim}
\newcommand{\dra}{\dashrightarrow}
\newcommand{\marnote}[1]{\marginpar{\textsc{\scriptsize #1}}}
\newcommand{\del}{\partial}
\newcommand{\HH}{H\mskip-2mu H}
\newcommand{\HT}{H\mskip-2mu T}
\newcommand{\HO}{H\Omega}
\newcommand{\bHH}{\overline{\HH}}
\newcommand{\bHT}{\overline{\HT}}
\newcommand{\remark}{\noindent\textbf{Remark: }}
\newcommand{\remarks}{\noindent\textbf{Remarks: }}
\newcommand{\question}{\noindent\textbf{Question: }}
\newcommand{\ii}{{\mathtt i}}
\newcommand{\smwedge}{{\scriptstyle{\wedge}}}
\newcommand{\EG}{\mathcal{EG}}
\newcommand\ske{\mathrm{asym}}	%anti-symmetrization
\newcommand{\bwed}{\bigwedge\nolimits}	%exterior product
\newcommand\p[1]{{{\mathbb P}^{#1}}} %Projective space
\newcommand{\field}[1]{\mathbb{#1}}
\renewcommand{\P}{\field{P}}
\newcommand{\A}{\field{A}}
\newcommand{\F}{\field{F}}
\renewcommand{\L}{\field{L}}
%% \theoremstyle{plain}
%% \newtheorem{theorem}{Theorem}[section]
%% \newtheorem{claim}[theorem]{Claim}
%% \newtheorem{lemma}[theorem]{Lemma}
%% \newtheorem{corollary}[theorem]{Corollary}
%% \newtheorem{proposition}[theorem]{Proposition}
%% \newtheorem{conjecture}[theorem]{Conjecture}
%% \theoremstyle{definition}
%% \newtheorem{definition}[theorem]{Definition}
%% \newtheorem{definition-theorem}[theorem]{Definition-Theorem}
%% \newtheorem{example}[theorem]{Example}
%% \newtheorem{notation}[theorem]{Notation}
%\theoremstyle{remark}
%\newtheorem{remark}[theorem]{Remark}
%\newtheorem{remarks}[theorem]{Remarks}
% This is used in order to have the heading in lowercase
%\renewcommand{\uppercase}{}
\renewcommand{\phi}{\varphi}
\newcommand{\vpic}[1]{\vcenter{\hbox{\epsfbox{#1.eps}}}}

